Evaluation of RIS-Enabled B5G/6G Indoor Positioning and Mapping using Ray Tracing Models

A Reconfigurable Intelligent Surface (RIS) can significantly enhance network positioning and mapping, acting as an additional anchor point in the reference system and improving signal strength and measurement diversity through the generation of favorable scattering conditions and virtual line-of-sight paths. In this paper, we present a comprehensive framework aimed at user localization and scatterer position estimation in an indoor environment with multipath effects. Our approach leverages beam sweeping through codebook-based beamforming at an 1-bit RIS to scan the environment, applies signal component extraction mechanisms, and utilizes a super-resolution algorithm for angle-based positioning of both connected users and scatterers. To validate the system's effectiveness, accurate 3D ray tracing models are employed, ensuring the robustness and effectiveness of the proposed approach in practical scenarios.

==> mycompress.tex <==
\setlength{\textfloatsep}{-5pt plus 3pt minus 2.0pt}		% space between last top float or first bottom float and the text
\setlength{\floatsep}{0pt plus 0pt minus 2.0pt}			% space left between floats
\setlength{\dblfloatsep}{-1pt plus 0pt minus 3.0pt}			% space left between floats
\setlength{\dbltextfloatsep}{-1pt plus 0pt minus 3.0pt}			% space left between floats
\setlength{\abovecaptionskip}{0pt plus 0pt minus 10pt}	% space above caption
\setlength{\belowcaptionskip}{0pt plus 0pt minus 3pt}	% space below caption
\setlength{\abovedisplayskip}{1pt plus 1pt minus 2pt}	% space before maths
\setlength{\belowdisplayskip}{1pt plus 1pt minus 2pt}	% space after maths

\renewcommand{\topfraction}{0.90}
\renewcommand{\bottomfraction}{0.90}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\textfraction}{0.02}
%extra compression with title spacings

\usepackage{titlesec}
\titlespacing*{\section}{0pt}{0pt plus 0pt minus 0pt}{0pt plus 1pt minus 2pt}
\titlespacing{\subsection}{0pt}{1pt plus 0pt minus 1pt}{0pt plus 0pt minus 1pt}
\titlespacing{\subsubsection}{0pt}{1pt plus 0pt minus 12pt}{1pt}

